Scalable Detection of Salient Entities in News Articles

News articles typically mention numerous entities, a large fraction of which are tangential to the story. Detecting the salience of entities in articles is thus important to applications such as news search, analysis and summarization. In this work, we explore new approaches for efficient and effective salient entity detection by fine-tuning pretrained transformer models with classification heads that use entity tags or contextualized entity representations directly. Experiments show that these straightforward techniques dramatically outperform prior work across datasets with varying sizes and salience definitions. We also study knowledge distillation techniques to effectively reduce the computational cost of these models without affecting their accuracy. Finally, we conduct extensive analyses and ablation experiments to characterize the behavior of the proposed models.

==> dataset_construction.tex <==
\section{Dataset Construction}
\subsection{Legacy Corpus for Entity Salience}
The legacy dataset includes data from almost 1400 articles for which titles and body text are available. Each document has salience annotations, on a scale of 1 to 10, for a set of candidate keyphrases (i.e., entity mentions and references) that were detected by the CAP boundary detection (i.e., keyphrase extraction) model, and keyphrases are linked to a Wikipedia entity where applicable. %Each phrase was labeled on a scale of one to ten for their saliency (one indicating the most salient) and is linked to a Wikipedia entity. 
After submitting a subset of these samples for rejudgement, we observed a large inconsistency between the rejudged and legacy labels (less than 50\% agreement), possibly due to the very granular label space. The other issue with the data was that the keyphrases were just a subset of salient entities, since the CAP keyphrase extraction model used to sample the judged phrases did not detect all salient phrases. This also means that improvements in the CAP keyphrase model may not lead to improvements in the evaluation metrics, since newly detected phrases would not have been judged for salience. The reliance on the existing CAP keyphrase model to create the legacy data meant that there was also no data available for training or evaluating an improved keyphrase model.

%We revisited the available data at the start of the project, primarily to ensure that we have a high quality dataset for unbiased model training/evaluation, and to ensure the guidelines and data are consistent. 

%(saliency label lower than four assumed positive, i.e., salient). 
%Since the distribution of data was affected with the quality of the keyphrase detection module, which may also change overtime. 

\subsection{Building a new Corpus for Entity Salience}
To address the shortcomings of the legacy dataset before starting a large-scale data labeling effort, we first simplified the label space to four classes, as defined in Table \ref{table:saleincy_scale_definitions}. Also, instead of providing candidate phrases to CAKE annotators, they were instead tasked with finding and labeling \textit{all} mentions of salient entities in articles based on the updated guidelines. For each entity, all the primary mentions with different surface forms are selected. As an example, in Figure~\ref{fig:sample_article}, \textcolor{blue}{\it Kevin de León}, \textcolor{blue}{\it Los Angeles city councilman} and \textcolor{blue}{\it De León}, are different surface forms of keyphrases that refer to the same entity. 
% \textbf{NEIL: it might be useful to give an example of what we mean by different surface forms here. Eliyar: added}
Each entity is also linked to its most relevant Wikipedia entity, if one exists. While this exhaustive labeling approach is uncommon in practice due to its higher annotation costs, having a reliable, accurate and comprehensive dataset was necessary to allow us to train and evaluate high quality models, while also providing future utility for other aspects of the entity salience pipeline, i.e., the same data can be used for training and evaluating models for keyphrase extraction and entity linking.
% \textbf{Maybe say a bit more here about how this dataset can be a general dataset for all 3 sub-problems, not just aboutness scoring. Eliyar: added to the end of paragraph.} 
%We capture co-references to a good extent in the dataset, since all primary mentions with different surface forms as well as more ambiguous mentions (references) of the entity are also specified. By co-references we mean all general phrases or words that cannot be related to any entity outside the scope of the article. 

Table \ref{table:sample_labeled} shows an example of the salient entities and their references labeled in an article by the CAKE team; an extract from the article itself is shown in  Figure \ref{fig:sample_article}. From Table \ref{table:sample_labeled}, we can see that each real-world entity is labeled with its canonical name as found in the article (i.e. \emph{Entity}) in addition to any non-canonical \emph{Aliases} and potentially ambiguous \emph{References}.  
%The Alias column includes other primary mentions of the entity in different surface forms that is considered as direct and important as the one in the Entity column. Reference column include more ambiguous references to the entity, which mostly includes co-references. Each entity and its references are indicated with the same color. 
Given that this labeling scheme produces \textit{all} mentions of primary and secondary salience entities and resolves them to Wikipedia identifiers, the resulting dataset is applicable to training keyphrase detection, salient entity scoring, as well as Wikipedia entity resolution models. 
% \textbf{NEIL: overall, this section looks pretty good, but it could definetly be improved to make it a little clearer. In particular, a brief clarification of what we mean be aliases/coreferences would help. We should probably also include definitions of the labels here too. Eliyar: added a sentence above on our definition of coreferences. the label definitions reference added above?}

To date, this ongoing effort has produced a corpus of approximately 6,000 articles with all salient entities and their references annotated. Our approach does not explicitly judge non-salient entities, however: for these we rely on CAP output and sample from entities that have no overlapping tokens (words) with phrases that have been explicitly labeled as salient. Since the CAKE team explicitly annotated \emph{all} salient entities in every article, any non-labeled phrases can be assumed to be non-salient. In addition to this, for our test partition of the data, any candidate phrases with a \emph{partial} match to a judged phrase was considered potentially ambiguous and sent to the CAKE team, in the form of document/label pairs, for secondary labeling. For the training partition of the data, such partial matching phrases were excluded from the training data (i.e. there were neither considered as positive or negative examples).
%salient entities and their linked Wiki entity does not match the ones for the salient entities. 

Table \ref{table:corpus_stats} shows the a summary of the new corpus alongside the legacy corpus. Since the focus of this work is updating models running on articles presented on Yahoo properties, which are primarily licensed from content partners, we initially focused on expanding annotations on licensed content. There is an ongoing effort to also create a new dataset for off-network articles that we also ingest into our systems. 
% \textbf{NEIL: It probably makes sense to include similar statistics about the legacy data, to give a sense of the differences between the two datasets. Also, the number of available phrases per document for negative sampling would be useful to add to the table, especially since this relates to the label imbalance during training. Eliyar: revised the table. The numbers for negative samples though are not reflecting the real statistics of the data, since the negatives are subsampled and also more affected by the length of the document used by the models}  

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{1.5pt}
\begin{tabular}{llll|l}
\hline
 \textbf{Entity} & \textbf{Alias} & \textbf{Reference} & \textbf{WikiEntity} & \textbf{Saliency} \\
\hline
 \textcolor{red}{Vicente Fernández} & \textcolor{red}{Vicente; Fernández; jefe de jefes} & \textcolor{red}{singer; legendary Mexican ranchera singer} & \textcolor{red}{Vicente\_Fernández} & \textcolor{red}{Excellent} \\
 \textcolor{violet}{Boyle Heights} & - & - & \textcolor{violet}{Boyle\_Heights,\_Los\_Angeles} & \textcolor{violet}{Excellent} \\
 \textcolor{orange}{Bailey Street} & - & - & - & \textcolor{orange}{Excellent} \\
 \textcolor{teal}{Boyle Heights Neighborhood Council} & - & \textcolor{teal}{neighborhood council; council} & - & \textcolor{teal}{Good} \\
 \textcolor{blue}{Kevin de León} & \textcolor{blue}{De León} & \textcolor{blue}{Los Angeles city councilman} & \textcolor{blue}{Kevin\_de\_León} & \textcolor{blue}{Good} \\
 \hline
\end{tabular}
\caption{Sample of labeled data. Different mentions are separated by ';'.}
\label{table:sample_labeled}
\end{table*}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.51\textwidth]{figures/sample_headline.png}
    \begin{minipage}{25em}{
    \textbf{
    Should \textcolor{red}{\underline{Vicente Fernández}} get a street in \textcolor{orange}{\underline{Boyle Heights}}? Question exposes a divided legacy}
    \newline
    \textcolor{violet}{\underline{Bailey Street}} passes Mariachi Plaza, …But the unassuming \textcolor{orange}{\underline{Boyle Heights}} street has become … the \textcolor{red}{\underline{legendary Mexican ranchera singer}} \textcolor{red}{\underline{Vicente Fernández}}, … But some members of the \textcolor{teal}{\underline{Boyle Heights Neighborhood Council}} were …\textcolor{blue}{\underline{ Kevin de León}}, the \textcolor{blue}{\underline{Los Angeles city councilman}} who represents the area, called \textcolor{red}{\underline{Fernández}} the “\textcolor{red}{\underline{jefe de jefes}}" in a motion … In a draft letter to \textcolor{blue}{\underline{De León}}, members of the \textcolor{teal}{\underline{neighborhood council}}'s Planning … said David Silvas, the \textcolor{teal}{\underline{council}}'s vice president … Carlos Montes, who serves on the \textcolor{teal}{\underline{neighborhood council}}, has grappled with \textcolor{red}{\underline{Fernández}}'s shortcomings.
}
    \end{minipage}
    \caption{Sample of labeled news article from Yahoo News frontpage. The Salient entities and their (co)references are specified with the same colors.}
    \label{fig:sample_article}
\end{figure}

\begin{table}[t]
\centering
\small
\begin{tabular}{l|l} 
\hline
 \textbf{1. Perfect (primary - single)}  &  the only most important entity \\
 \textbf{2. Excellent (primary - multiple)} & equally important primary entities \\
 \textbf{3. Good (secondary)} & relevant but not considered primary \\
 \textbf{4. Fair or Bad} & hardly relevant or not relevant \\
 \hline
\end{tabular} 
\caption{Entity saliency scales/definitions.}
\label{table:saleincy_scale_definitions}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{l|l|l|l|l} 
\hline
\  & \multicolumn{3}{c}{\textbf{New Dataset}} & \multirow{1}{*}{\textbf{Legacy}} \\
\  & \textbf{Train} & \textbf{Valid.} & \textbf{Test} &  \\
\hline
 \#documents  & 3757 & 432 & 1193 & 222 \\ % 1367 \\
 \#ave. salient entities per doc. & 4.36 & 5.05 & 5.10 & 4.07 \\ % 4.94 \\
 \#Perfect & 1446 & 143 & 378 & 75 \\ % 551 \\
 \#Excellent & 6127 & 707 & 1972 & 433 \\ % 1045 \\
 \#Good & 4078 & 471 & 1323 & 339 \\ % 4281 \\
 \#Bad & 78447 & 9246 & 25424 & 5134 \\ % 8620 \\
 \hline
\end{tabular} 
\caption{Current corpus statistics of the annotated salient entities for the licensed data.}
\label{table:corpus_stats}
\end{table}



